CompactFlowNet: Efficient Real-time Optical Flow Estimation on Mobile Devices

We present CompactFlowNet, the first real-time mobile neural network for optical flow prediction, which involves determining the displacement of each pixel in an initial frame relative to the corresponding pixel in a subsequent frame. Optical flow serves as a fundamental building block for various video-related tasks, such as video restoration, motion estimation, video stabilization, object tracking, action recognition, and video generation. While current state-of-the-art methods prioritize accuracy, they often overlook constraints regarding speed and memory usage. Existing light models typically focus on reducing size but still exhibit high latency, compromise significantly on quality, or are optimized for high-performance GPUs, resulting in sub-optimal performance on mobile devices. This study aims to develop a mobile-optimized optical flow model by proposing a novel mobile device-compatible architecture, as well as enhancements to the training pipeline, which optimize the model for reduced weight, low memory utilization, and increased speed while maintaining minimal error. Our approach demonstrates superior or comparable performance to the state-of-the-art lightweight models on the challenging KITTI and Sintel benchmarks. Furthermore, it attains a significantly accelerated inference speed, thereby yielding real-time operational efficiency on the iPhone 8, while surpassing real-time performance levels on more advanced mobile devices.

==> sections/06_supplementary_materials.tex <==
\section{Supplementary Material}

\subsection{Computational profiling}
Measurement of running time across lightweight optical flow models and various deployment devices is provided, see Table~\ref{table_running_time}. Performance is measured directly on device for all of the listed methods, i.e. all of the models were implemented in PyTorch and converted to TFLite for on-device inference. Latency is calculated as an average over 100 runs performed after 100 warm-up runs. Inference capabilities of the models under investigation are demonstrated using input images of 512x512, 436x1024 (the resolution of Sintel images), and 1080x1920 (Full HD) resolutions. This strategy effectively represents a range of computational demands, thereby providing a comprehensive analysis of model performance under varying operational conditions.\footnote{Theoretical latency values for several models in Table~\ref{table_main_results_speed} should be substituted with real on-device measurements listed in the Supplementary materials section.}

\begin{table}[!htb]
\caption{Running time (ms), iPhone 8 | iPhone XR | iPhone 12 | iPhone 14 Pro}
\label{table_running_time}
\centering
\small
\begin{threeparttable}
\begin{tabular}{l p{4cm} p{4cm} p{4cm}} 
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Input resolution}  \\
\cmidrule(lr){2-4}
 & \multicolumn{1}{c}{512x512} & \multicolumn{1}{c}{436x1024} & \multicolumn{1}{c}{1080x1920} \\
\midrule  
PWC-Net+                  & \multicolumn{1}{c}{212 |	115 |	114 |	62}	& \multicolumn{1}{c}{343 |	198 |	154 |	102} & 	\multicolumn{1}{c}{1787 |	1440 |	875 |	474} \\
PWC-Net-small             & \multicolumn{1}{c}{96 |	58 |	45 |	\textbf{30}\tnote{a}} &	\multicolumn{1}{c}{167 |	103 |	72 |	51} 	& \multicolumn{1}{c}{926 |	553 |	406 |	235} \\
FDFlowNet                 & \multicolumn{1}{c}{127 |	72 |	53 |	\textbf{37}}	& \multicolumn{1}{c}{218 |	125 |	93 |	63} &	\multicolumn{1}{c}{1187 |	658 |	504 |	292} \\
FastFlowNet               & \multicolumn{1}{c}{60 |	\textbf{36} |	\textbf{32} |	\textbf{16}} &	\multicolumn{1}{c}{91 |	54 |	\textbf{41} |	\textbf{28} } &	\multicolumn{1}{c}{433 |	248 |	214 |	137} \\
CompactFlowNet            & \multicolumn{1}{c}{\textbf{40} |	\textbf{26} |	\textbf{19} |	\textbf{13}} &	\multicolumn{1}{c}{71 |	\textbf{41} |	\textbf{34} |	\textbf{23} } &	\multicolumn{1}{c}{349 |	209 |	179 |	114} \\
\bottomrule
\end{tabular}
\begin{tablenotes}
      \small
      \item[a] Running times indicated in bold font correspond to latency compatible with real-time inference.
\end{tablenotes}
\end{threeparttable}
\end{table}

\begin{table}[!htb]
\caption{Peak memory footprint (MB)}
\label{table_memory_footprint}
\centering
\small
\begin{tabular}{l c c c} 
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Input resolution}  \\
\cmidrule(lr){2-4}
 & 512x512 & 436x1024 & 1080x1920 \\
\midrule  
PWC-Net+                  & 239 &	327 &	879 \\
PWC-Net-small             & $\underline{151}$ &	$\underline{205}$ &	$\underline{529}$ \\
FDFlowNet                 & 185 &	257 &	659 \\
FastFlowNet               & 261 &	271 &	535 \\
CompactFlowNet            & \textbf{118} &	\textbf{146} &	\textbf{370} \\
\bottomrule
\end{tabular}
\end{table}

CompactFlowNet exhibits superior speed on all evaluated devices compared to other lightweight approaches. With respect to the quality metrics estimated on KITTI 2015 and Sintel test sets, its performance aligns closely with that of FDFlowNet and PWC-Net+, despite these latter models being significantly more time-consuming on mobile devices. Furthermore, PWC-Net-small demonstrates a slower speed along with a lower quality output when compared to CompactFlowNet. FastFlowNet, while presenting a satisfactory inference speed, underperforms on the Sintel test and is slower on mobile devices compared to CompactFlowNet by a margin of 20-50$\%$. Remarkably, CompactFlowNet is the pioneer in providing online inference speed on iPhone 8 and iPhone XR, handling relatively high resolutions of 512x512 and 436x1024 respectively. Despite online inference on larger resolutions posing a significant challenge, CompactFlowNet successfully achieves nearly 10 FPS on iPhone 14 Pro when processing FullHD resolution input images.

Moreover, when it comes to memory usage, CompactFlowNet surpasses other lightweight optical flow models, as illustrated in Table~\ref{table_memory_footprint}. Although the specific memory demands are dependent on the application, CompactFlowNet's reduced memory consumption increases its adaptability and suitability for various uses. With its superior attributes, including less memory usage, quicker inference speed, and higher quality, CompactFlowNet stands out as the optimal selection for real-world applications.





\subsection{Visual comparison}
See Figure~\ref{fig:figure_results_sintel_clean}, Figure~\ref{fig:figure_results_sintel_final} and Figure~\ref{fig:figure_results_kitti} to visually review performance of different lightweight models.
\begin{figure}[!htb]
  \centering
  \includegraphics[scale=0.17]{figures/results_Sintel_clean.png}
  % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Visualized results on Sintel Clean test set.}
  \label{fig:figure_results_sintel_clean}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[scale=0.17]{figures/results_Sintel_final.png}
  % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Visualized results on Sintel Final test set.}
  \label{fig:figure_results_sintel_final}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[scale=0.3]{figures/results_KITTI.png}
  % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Visualized results on KITTI 2015 test set.}
  \label{fig:figure_results_kitti}
\end{figure}

